FAILS: A Framework for Automated Collection and Analysis of LLM Service Incidents

Large Language Model (LLM) services such as ChatGPT, DALLE, and Cursor have quickly become essential for society, businesses, and individuals, empowering applications such as chatbots, image generation, and code assistance. The complexity of LLM systems makes them prone to failures and affects their reliability and availability, yet their failure patterns are not fully understood, making it an emerging problem. However, there are limited datasets and studies in this area, particularly lacking an open-access tool for analyzing LLM service failures based on incident reports. Addressing these problems, in this work we propose FAILS, the first open-sourced framework for incident reports collection and analysis on different LLM services and providers. FAILS provides comprehensive data collection, analysis, and visualization capabilities, including:(1) It can automatically collect, clean, and update incident data through its data scraper and processing components;(2) It provides 17 types of failure analysis, allowing users to explore temporal trends of incidents, analyze service reliability metrics, such as Mean Time to Recovery (MTTR) and Mean Time Between Failures (MTBF);(3) It leverages advanced LLM tools to assist in data analysis and interpretation, enabling users to gain observations and insights efficiently. All functions are integrated in the backend, allowing users to easily access them through a web-based frontend interface. FAILS supports researchers, engineers, and general users to understand failure patterns and further mitigate operational incidents and outages in LLM services. The framework is publicly available on https://github.com/atlarge-research/FAILS.

==> sections-import/1-introduction2.tex <==
\section{Introduction}

Large Language Models (LLMs) are transforming industries by automating tasks such as customer service, content generation and decision-making processes, and aid scientific research\cite{Arman2023Sep}. These systems operate as highly complex distributed services, involving geographically dispersed components for training, inference, and user interaction\cite{chkirbene2024large}. However, their complexity makes LLM services prone to failures in their infrastructure, software and their external dependencies. Failures and outages have major costs for users relying on LLM services and thus can cause a significant degradation in customer loyalty, which explains why even the largest providers issue public apologies after a system-wide outage \cite{observability_report, x_postopenai}. Understanding and mitigating these failures is a critical challenge for maintaining the reliability and trustworthiness of these systems\cite{yu2024survey}.

\subsection{Motivation} 

Currently, tools for analysing incidents and outages of services in distributed systems offer only partial functionality. Sites such as \href{https://smartbear.com/product/alertsite/}{SmartBear AlertSite}\cite{SmartbearAlertSite}, \href{https://uptimerobot.com/}{UptimeRobot}\cite{UptimeRobot} and \href{https://www.pingdom.com/}{Pingdom}\cite{Pingdom} offer enterprise monitoring services, but are closed-source and aimed at business customers and system administrators. \href{https://downdetector.com/}{Downdetector}\cite{Downdetector} offers real-time problem and outage monitoring of public websites, but as a user driven site lacks comparative tools and in-depth root-cause analysis, as well as the ability to select and compare different services from one provider. 

This leaves the self-reported status pages of the individual providers. While publicly available, they lack standardization and analysis tools, complicating efforts to perform comparative analyses between different providers and services. Although some work has been done to collect and investigate failures from these pages \cite{ReferenceWork}, there remains a market gap for tools that integrate data scraping, analysis, and visualization in a unified, open-source framework for researchers, small business owners looking for an optimal solution, and the interested public.

\subsection{Our Solution}

To address this need, we present a \textit{Framework for Analysis of Incidents and Outages of LLM Services (FAILS)}, which is designed to:

\begin{enumerate}
    \item Automatically scrape, process, clean and store failure data from LLM provider status pages;
    \item Visualize temporal failure trends, correlations and recovery patterns;
    \item Perform statistical evaluations of reliability metrics, such as Mean Time to Recovery (MTTR) and Mean Time Between Failures (MTBF);
    \item Integrate LLM-assisted methods to provide contextual insights into analysis results;
    \item Present the user with an easy to use web-based interface to access all tools
\end{enumerate}

The remainder of this paper provides a brief background on LLMs, their issues and the requirements for an effective analysis tool. We then describe the architecture of the FAILS system, highlighting its core functionalities and implementation, and present a few selected experimental results obtained using it. Finally, we discuss potential future improvements and additional functionalities that could be added to this open-source project.



 










==> sections-import/2-background2.tex <==
\section{Background}
\subsection{The Complexity of LLM Services}
LLM services are complex distributed systems designed to process and generate text, leveraging vast amounts of data and computational resources in the process. From a distributed systems perspective, LLM services consist of multiple interconnected components, including model storage, training pipelines, inference engines, and data-handling subsystems, as well as interfaces to allow users to interact with them. All of these components operate across geographically dispersed machines and must work cohesively to support the immense compute and memory requirements of training and serving models \cite{Brakel2024ModelPO, Duan2024EfficientTO}.

This complexity and size comes with significant challenges, including ensuring scalability as demand and models grow, managing energy consumption, and handling failures in their distributed components. These challenges are further compounded by external dependencies such as third-party APIs, load balancers, and content delivery networks. Analysing service failures is a complex task, as self-reported incidents are often limited by company policies, and even the companies themselves may struggle to immediately identify the nature or origin of a failure. A tool to analyse failures must therefore be able to deal with dynamic data structures, offer granular insights and be accessible (open-source).

\subsection{Requirements for a Failure Analysis Tool}

\begin{enumerate}[label=\textbf{FR\arabic*}]
    \item \textbf{Data Collection and Processing}: The system must be capable of automatically scraping incident and outage data from multiple service providers. Given the distributed nature of these services, the pipeline must handle potential challenges like incomplete or changing data structures.
    \item \textbf{Data Cleaning and Storage}: The collected data must be cleaned to ensure it is consistent and saved in a structured format (e.g., CSV). This step is essential to facilitate downstream analysis. Cleaning includes handling missing values, standardizing date-time formats, and ensuring compatibility across datasets from different providers.
    \item \textbf{Failure Recovery Model}: The system must be able to analyze failures using common metrics such as Mean Time to Recovery (MTTR) and Mean Time Between Failures (MTBF). The failure recovery model should allow users to identify trends, compare metrics across providers, and evaluate how quickly services recover from disruptions \cite{gamell2014exploring, avizienis2004basic}.
    \item \textbf{Temporal and Co-occurrence Analysis}: The system should support the exploration of failure patterns over time (temporal analysis) and identify relationships between failures (co-occurrence analysis).
    \item \textbf{Visualization and Reporting}: The results of the analysis must be presented in an accessible and automated format. This includes tables, figures (e.g., time series, bar charts), and textual summaries of key metrics.
\end{enumerate}


\begin{enumerate}[label=\textbf{NFR\arabic*}]
    \item \textbf{Accessible, web-based interface}: To ensure usability across a broad audience, including non-technical users, the system should provide a modern, responsive, and intuitive web-based interface. This aligns with the principle of abstraction and accessibility in distributed systems by enabling users to interact with advanced data processing without specialized knowledge. This also facilitates easy distribution and deployment via standard web technologies.
    \item \textbf{Reliability and Fault Tolerance}: The system should consistently operate without unexpected downtime or errors, particularly during data scraping and analysis. Failures in this context could arise from new or inconsistent data formats from service providers. While it is impossible to foresee all new possible errors, implementing mechanisms for to ensure fault tolerance, such as retry logic, validation checks for incoming data and user level error messages, ensures robustness and reliability\cite{isukapalli2024systematic}.
    \item \textbf{Performance and Scalability}: Ensuring it can run on general web servers and consumer level machines well is essential when it comes effective distribution. Future proofing the application by ensuring elasticity (vertical and horizontal scalability) is essential in the rapidly developing field of LLMs. Using generalised methodologies to scrape the data facilitates adding more services as they appear in the market, and making sure longer time-frames can be supported as well adds value to the application.
    \item \textbf{Analysis support using LLMs:} Integrating the capabilities of LLM chatbots into the analysis pipeline adds the possibility to provide contextual insights into failure patterns. This includes generating informed prompts to assist users in root cause analysis and help understand more technical concepts such as the failure models used.
    % \item (Security and Data Privacy)
\end{enumerate}


\subsection{Theoretical Background for Failure Analysis}
\label{sec:theoback}
\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/frm.png}
    \caption{\textbf{Conceptual overview of the failure recovery model.} The model outlines the five key stages in incident management, visualising them in sequential order: Investigating, Identified, Monitoring, Resolved, and Postmortem.}
    \label{fig:frm}
\end{figure}


The figures presented in this paper display the results of various statistical analyses, most of which are grounded in a Failure Recovery Model. This model provides a systematic framework to analyze how providers handle incidents, offering insights into fault tolerance and resilience \cite{gamell2014exploring, avizienis2004basic}.



\textbf{Failure Recovery Model:} The model comprises five key stages that describe the lifecycle of incident handling (also visualised in Figure \ref{fig:frm}):
\begin{itemize}
    \item \textbf{Investigating Status (S1):} The operational team begins analyzing the issue immediately after it is detected.
    \item \textbf{Identified Status (S2):} The root cause of the incident is identified.
    \item \textbf{Monitoring Status (S3):} A fix is implemented, and the system is monitored to ensure the resolution is effective.
    \item \textbf{Resolved Status (S4):} The incident is considered resolved, and normal operations resume.
    \item \textbf{Postmortem Status (S5):} A detailed summary of the incident is prepared to analyze the root cause and suggest measures to prevent recurrence.
\end{itemize}

This model enables the calculation of several key performance metrics:
\begin{itemize}
    \item \textbf{MTBF (Mean Time Between Failures):} This metric calculates the average time between two consecutive failures for a provider. It serves as an indicator of how fault-tolerant the provider’s system is.
    \item \textbf{MTTR (Mean Time to Recovery):} Derived from the failure recovery model, MTTR measures the total time taken to resolve a failure, encompassing the period from investigation (S1) to resolution (S4). It provides insights into how quickly a provider can respond to and rectify failures.
\end{itemize}

Additionally, other metrics derived from the analysis are discussed:
\begin{itemize}
    \item \textbf{Co-occurrence of Failures per Provider:} This metric quantifies the number of services affected simultaneously during a failure for each provider. It highlights service interdependencies and provides insights into the potential benefits of compartmentalization and dependency separation.
    \item \textbf{Impact Classification Distribution:} Although the largest providers utilize a standardized framework to classify the severity of failures, variations exist in their classification tendencies. These differences reflect the providers' operational priorities and reporting practices.
\end{itemize}

==> sections-import/3-system-design2.tex <==
\section{System design}


In order to address the requirements, we developed a system to facilitate the analysis of incidents and outages of Large Language Models services. Aptly named \textit{FAILS (Framework for Analysis of Incidents and Outages of LLM Services)}, it provides a web-based interface for automatically scraping the data from the providers and interacting with it in the form of tables, plots and text based outputs. Without loss of generality, we chose services from OpenAI (ChatGPT\cite{OpenAIChatGPT}, API service\cite{OpenAIAPI}, DALL-E\cite{OpenAIDALLE} and Playground\cite{OpenAIPlayground}), Anthropic (Claude\cite{AnthropicClaude}, API\cite{AnthropicAPI}, and Console\cite{AnthropicConsole}), CharacterAI\cite{CharacterAI} and StabilityAI (RestAPI\cite{StabilityRESTAPI}, gRPC API\cite{Stabilitygrpc} and Stable Assistent\cite{StabilityAssistent}) to demonstrate the viability and effectiveness of our solution.




\subsection{System architecture}
\textit{FAILS} follows a modern client-server architecture. The frontend is built in React.js \cite{ReactJS} with Material UI \cite{MaterialUI} components, which provide a modern, responsive and intuitive user interface. This enables non-technical users to access the advanced data processing and analysis pipeline effectively and developers to easily modify the code of \textit{FAILS}, since React is the most popular JavaScript framework \cite{ReactPop} and Material UI is built on Google's design language.

The backend encapsulates the data scraping, processing and analysis functionality with a Flask-based server, which is lightweight, popular and scalable \cite{Flask}. Figure \ref{fig:architecture} gives insight into the architecture of the application. 



\begin{figure}[h!]
    \centering
    \includegraphics[width=0.82\linewidth]{figures/architecture2.png}
    \caption{\textbf{Architecture of \textit{FAILS}}: structural overview of the application, consisting of scraping functionality, the tabular data display, plot visualisation and AI tools in the backend, which are all accessible from a React-based web interface. The scraping pipelines are shown separately and generate a final CSV, which process powers all other functionality.}
    \label{fig:architecture}
\end{figure}




\subsection{Features}

The requirements set in the previous steps are addressed by the implementation of the following features:

\begin{enumerate}[label=\textbf{F\arabic*}]
    \item \textbf{Data scraping pipeline}\\
    The data scraping pipeline uses headless Chrome browsers through Selenium WebDriver \cite{Selenium} to systematically extract incident data from the service providers \cite{StatusOpenAI, StatusAnthropic, StatusCharacterAI, StatusStabilityAI}. It is widely supported, handles complex authorisation well and enables dynamic data retrieval by simulating user interactions, such as clicks and scrolls. The scraper utilizes explicit WebDriverWait conditions to ensure proper loading of dynamic content and implements retry mechanisms to handle potential stale elements or network issues.
    
    First, the incident history page is loaded to obtain a list, from which it expands the information on the individual incidents and is able to extracts the attributes and metadata. This includes the title, impact level and a colour which represents the severity. To ensure uniqueness, an ID is assigned to each incident, which is either derived from the URL (OpenAI, Anthropic and CharacterAI) or generated using UUID in the case of StabilityAI. Additionally, we extract granular timeline information, such as start and end time for the entire failure and, where available, for the individual stages (see section \ref{sec:theoback}) of failure recovery.

    As OpenAI, Anthropic and CharacterAI use status pages based on \textit{Atlassian Statuspage}\cite{Atlassian2025Jan}, the page and data structure is similar and can be handled within one pipeline (see previous work done by X. Chu et al.\cite{ReferenceWork}). The scraped data undergoes a transformation process, where timezones are normalised to UTC. Service identification is handled through a detailed parsing mechanism that recognizes both explicit service mentions and implicit references in the incident descriptions. The system then processes and unifies the incident updates, which are stored as JSON strings, to categorize the different incident stages. The data is saved to a temporary CSV file.

    As for StabilityAI, the scraper is based on \textit{Instatus} \cite{Instatus} and is structured differently. Aside from the page structure and location of metadata, StabilityAI has a unique set of services (REST API, gRPC API, Stable Assistant) that require specific detection logic. While the core scraping process is similar, we needed to ensure that the impact levels, colours and failure messages are consistent, and do this through a careful translation process. This cleaned data is also saved to a temporary CSV file.
    
    Before merging the data, the system performs thorough validation checks on both raw and transformed data, ensuring data integrity and structural consistency. The final processed data is saved to a combined CSV, with careful handling of file backups, temporary files and restore operations to prevent data corruption. The system maintains separate archives for raw data from each provider while combining them into a unified, normalized format in the final output file. This standardized file supports analysis and visualization, aligning records across services based on timestamps and incident IDs. The approach ensures the pipeline achieves both reliability and scalability, addressing FR1, FR2, NFR2 and NFR3.

    The entire process can be launched from a single script, which also handles errors and ensures unique data entries. Thus, integration in the front end is simplified to a single API endpoint that triggers the entire scraping process and handles errors and retries gracefully.
    
    \item \textbf{Display of the data as table}\\
    The CSV format the data is saved in enables the effective display using a table, such as in Material-UI's \textit{DataGrid}\cite{MUIDataGrid}. We used this to display select properties in a way that users can easily find information on the latest recorded failures. Through color coding, users can quickly identify services and impact levels, and read the precise error messages as reported by the providers - all on one page. Sorting by dates, durations, providers and impact levels aids the overview and helps investigate and verify analysis results. Additionally, the data scraping pipeline can be started from a button here, which automatically updates the table. This addresses FR5.
    \item \textbf{Automated plotting}\\
    Our "Dashboard" page has the functionality to select a time-frame and a set of individual services from the dataset and plot metrics from this subset of data in an automated fashion (addresses FR3 and FR5). The generated plots can easily be downloaded individually or in bulk as high-resolution PNGs, ready for sharing or for the use in papers and presentations. A complete list of the plots generated by \textit{FAILS} can be found in the appendix, table \ref{tab:plot_overview}.
    \item \textbf{Plot analysis using LLM-assisted methods}\\
    To aid the interpretation of the generated plots, especially for a non-scientific audience, we implemented an automatic analysis pipeline, which addresses NFR4. It enables users to generate an automatic analysis of the currently individual plots. This works by sending the image to an LLM service (in our test case, the API of OpenAI's \textit{gpt-4o-mini}), packed in a prompt informed by the knowledge of the individual graph. For example:
    \begin{quote}
            \textit{Analyse this impact level distribution \textsc{\{date\_range, selected\_services, image\}}. Knowing that the impact levels are defined as \textsc{\{impact\_definition\}}, and we have calculated following metrics \textsc{\{statistical\_measures (mean, median, number of incidents,...)\}}, focus on the differences in the distributions between the services!}
    \end{quote}
    Additional prompts ensure a structured output of a predefined length, which enables us to format and show the response in the front-end. Additionally, we implemented an option to analyse all the plots in bulk, by passing the entire set of generated plots with a prompt, telling the model to focus on the most significant findings.
    \item \textbf{Interacting with the dataset using LLMs}\\
    The aforementioned automated plot analysis has its limitations as it relies on predefined prompts and pre-calculated metrics. To add a more dynamic way of interacting with the data, we fed a cleaned version of the dataset and metrics on it to the LLM API. This way, the user can use a chatbot interface to ask targeted questions about the dataset, such as the number of incidents, the time range of the dataset or causes of individual events. Especially in conjunction with the data table and the generated plots, this enables deep insight into the data. Further experimenting with different prompting paradigms could result in more informative outputs by the LLM\cite{white2023prompt}.
    
    \item \textbf{Functionality wrapped in a web interface}\\
    All of this functionality is neatly wrapped in a web-app interface (NFR1), which includes modern functionality such as theming and responsiveness. The individual functions mentioned above are arranged in a sidebar menu, which is clean and easily accessible and includes a page with information on the project.
\end{enumerate}








\subsection{Design process}
The design process followed a structured approach to ensure clarity, collaboration, and effective execution. The first step involved maintaining a comprehensive to-do list to track progress and prioritize tasks, which were discussed with our TA in weekly meetings. We began by analysing the problem from a high-level perspective, then setting out the functional and non-functional requirements based on the problem and user needs. We checked the market for similar tools too, such as Grafana\cite{Grafana} for monitoring Distributed Systems, Datadog\cite{Datadog} for incident tracking, and Splunk\cite{Splunk} for log analysis, as well as the tools mentioned in the introduction. These examples provided inspiration and highlighted gaps in existing solutions that our system could address. A working design document was created to outline the system architecture, core components, and implementation strategy, which served as a reference throughout the development process.

Tasks were divided based on team members' areas of expertise to maximize efficiency. Regular meetings and iterative feedback loops ensured that we remained on track, allowing adjustments to the design as ideas emerged. Thus, we were able to successfully translate the initial requirements into a robust and functional system.

==> sections-import/4-experimental-results2.tex <==
\section{Experimental Results}
This section presents the findings of our statistical analyses based on the theoretical framework introduced earlier and is meant to demonstrate a use case of our system. The analyses done highlight key differences in the failure recovery processes and resilience of the providers studied. Figures \ref{fig:co-occurence}, \ref{fig:mtbf}, \ref{fig:mttr} are inspired by previous work from X. Chu et al \cite{ReferenceWork}.

\subsection{Mean Time Between Failures (MTBF)}
Figure \ref{fig:mtbf} shows the Cumulative Distribution Function (CDF) of the Mean Time Between Failures (MTBF) for each provider. CharacterAI and StabilityAI exhibit longer MTBFs compared to OpenAI and Anthropic, which is likely due to the higher complexity and user demand faced by the latter two providers. In contrast, smaller user bases and simpler system designs likely contribute to the extended MTBFs of CharacterAI and StabilityAI.

\begin{figure}[H]
    \centering
    \includegraphics[trim=30 9 2 8, clip, width=1\linewidth]{figures/MTBF_CDF.png}
    \caption{\textbf{Cumulative Distribution Function (CDF) of the Mean Time Between Failures (MTBF) for Each Provider from February 2021 to December 2024} A steeper CDF indicates that MTBF values are less evenly distributed, while a distribution function shifted further to the right signifies longer times between failures for the provider. Notably, CharacterAI and StabilityAI exhibit longer MTBFs and less steep CDFs compared to OpenAI and Anthropic.}
    \label{fig:mtbf}
\end{figure}

\subsection{Mean Time to Recovery (MTTR)}
The CDF of the Mean Time to Recovery (MTTR) for each provider is presented in Figure \ref{fig:mttr}. StabilityAI shows shorter recovery times than OpenAI, Anthropic, and CharacterAI. This outcome suggests more efficient recovery mechanisms and a smaller operational scale that facilitates fault-tolerant systems.

\begin{figure}[H]
    \centering
    \includegraphics[trim=30 9 2 8, clip, width=1\linewidth]{figures/MTTR_CDF.png}
    \caption{\textbf{Cumulative Distribution Function (CDF) of the Mean Time to Recovery (MTTR) for Each Provider  from February 2021 to December 2024}. A steeper CDF indicates less evenly distributed MTTR values, while a distribution function shifted further to the right represents longer recovery times for the provider. StabilityAI exhibits a left-shifted CDF compared to the other three, indicating significantly shorter recovery times.}
    \label{fig:mttr}
\end{figure}

\subsection{Co-Occurrence of Failures}
Figure \ref{fig:co-occurence} highlights the number of services affected simultaneously during failures for each provider. Anthropic frequently experiences failures affecting multiple services, suggesting significant interdependencies among its systems. In contrast, OpenAI and StabilityAI tend to experience failures that impact only one service, indicating better compartmentalization and reduced cascading risks.

\begin{figure*}[h!]
    \centering
    \includegraphics[width=0.32\textwidth]{figures/Impact_LevelA.png}
    \includegraphics[width=0.32\textwidth]{figures/Impact_LevelO.png}
    \includegraphics[width=0.32\textwidth]{figures/Impact_LevelS.png}
    \caption{\textbf{Co-occurrence of failures across services for each provider from February 2021 to December 2024}. 
    The subplots illustrate the number of services impacted during a failure for each provider. 
    \textbf{(a)} For Anthropic, failures most frequently impact all three services simultaneously. 
    \textbf{(b)} For OpenAI, failures tend to impact a single service more often than multiple services. 
    \textbf{(c)} For StabilityAI, failures predominantly affect only one service at a time.}
    \label{fig:co-occurence}
\end{figure*}

\subsection{Impact Level Classifications}
Figure \ref{fig:impact_level_dist} depicts the distributions of failure impact level classifications for each provider on a 1–5 severity scale. OpenAI and Anthropic exhibit similar distributions, while CharacterAI tends to classify failures as highly severe. StabilityAI’s less granular classification system, with a concentration around a mean score of 3, likely reflects its smaller operational scope and differing reporting standards.

\begin{figure*}[h!]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/impact_level_distribution_February 2021 - December 2024.png}
    \caption{\textbf{Distributions of Impact Level Classifications per Provider (February 2021 to December 2024):} The figure illustrates the classification of failures by each provider on a 1–5 severity scale. OpenAI and Anthropic exhibit similar distributions, while CharacterAI shows more failures as highly severe. StabilityAI shows a concentrated distribution around the mean score (3), with relatively few classifications at higher or lower values, indicating a less granular classification system. This analysis highlights the discrepancies in reporting between the providers, differences in reporting standards influence the direct comparison.}
    \label{fig:impact_level_dist}
\end{figure*}

\subsection{Summary of Findings}
The findings underscore notable differences among providers in terms of fault tolerance, recovery efficiency, and classification practices. StabilityAI demonstrates efficient recovery capabilities and compartmentalized service design, whereas OpenAI and Anthropic face challenges in maintaining long MTBFs due to their larger scale. Impact classification distributions highlight the varying operational priorities and reporting approaches of the providers.



==> sections-import/5-discussion2.tex <==
\section{Discussion}

The FAILS framework significantly streamlined the execution of our analytical experiments by integrating data processing, visualization, and analysis workflows. The scraping pipeline ensured that all data we investigated was up-to-date and reliable across providers, enabling the comparative study of metrics such as MTBF, MTTR, and failure co-occurrence patterns. 

The interactive dashboard allowed for dynamic exploration of these metrics. For example, the automated CDF visualizations provided insights into variations in recovery times and the distribution of impact classifications, while the LLM-assisted contextual analysis generated detailed interpretations of provider-specific behaviors, such as differences in system resilience and recovery mechanisms.

The tool also facilitated experimenting with visualizations. For instance, we were able to test whether showing all providers on the same CDF plot was informative or if it made the plots too crowded and thus better suited for individual provider plots. With \textit{FAILS}, this comparison took only a few seconds and a few button switches, whereas for a non-technical user, such changes would require significant time to refactor.

This modular design reduced manual effort, enabled efficient cross-provider comparisons, and provided actionable insights into the failure dynamics of large-scale distributed systems.


\subsection{Limitations and future work}
Our system provides a foundation for the effective analysis of LLM failures. Due to its modular setup and the usage of modern frameworks and components, it leaves ample opportunity for developers to further scale and improve it. 

Adding real-time analysis, collecting data as the failures occur, would open the door to more in-depth features, such prediction the recovery time of a failure upon the first report of downtime. A proposed way of doing this is to treat all known properties of the failure at hand (such as provider, service, geographical location, time of the day, availability of other similar services, statistics of historical data etc.) as a feature vector and predict the Time to Resolve using a Transformer Architecture.

The LLM analysis features could be further improved by in-depth testing and validation. More refined prompts and adding more knowledge about the systems and historical context as it becomes available could improve the quality of the responses. A Retrieval-Augmented Generation (RAG) system would add value, adding a knowledge database to the context. Also, especially in the case if real-time data is added, utilising local models instead of APIs of commercial ones would boost the fault tolerance of our system, ensuring \textit{FAILS} stays fully functional even while it records failures.

Another feature worth exploring could include an in-depth geographical analysis, comparing the incidents across different countries. One way of doing this is extracting user-reported outages on Downdetector, which has a local site for 50 countries \cite{Downdetector}. Apart from using the enterprise API, this would require scraping the number of outages from dynamically generated graphs, something we weren't able to do within our timeframe with our current toolset (Selenium). Achieving this would also enable comparative analysis between the provider-reported and user-reported incidents. This would help minimise errors in the reporting and help understand reports maimed by company policy.

Moving away from the concept of downtime, further analysis could yield interesting results on performance degradation failures, when partial failures influence the quality of output from an LLM service. For example, a failure in a data preprocessing subsystem might result in incomplete or noisy input being fed into the model, leading to nonsensical or lower-quality text generation. Similarly, a partial failure in the inference engine, for example reduced computational capacity on certain nodes, could increase response latency or force the system to use fallback models that produce less accurate results. By systematically analysing metrics like output coherence, response accuracy, and latency one could quantify degradation. This would provide a deeper understanding of how such failures impact user experience and offer insights into fine-tuning fault tolerance mechanisms.

As new LLM providers emerge, \textit{FAILS} should be updated to include additional services. For example, services like Sora, which appeared after this project’s timeline, appear in the error messages but can't automatically assigned to a service, should be incorporated into future iterations. Ideally, this would involve a dynamic integration system, where minimal manual work is needed to incorporate new providers and services. Implementing distributed databases or multi-server architectures could ensure that \textit{FAILS} remains performant as datasets grow in size or complexity.




==> sections-import/6-conclusion2.tex <==
\section{Conclusion}
\textit{FAILS} represents a step towards addressing the challenges of failures of complex LLM ecosystems. By combining automated data scraping, advanced analytics, and intuitive visualizations within a modular, web-based interface, \textit{FAILS} bridges critical gaps in understanding and mitigating service disruptions. Its potential for real-time data integration, predictive modelling, and deeper geographical and user-reported incident analysis emphasises the framework’s adaptability.

By providing actionable insights into failure trends and recovery patterns, \textit{FAILS} lays a foundation for improved reliability across LLM platforms, empowering users to make informed decisions. As the adoption of LLMs continues to grow, \textit{FAILS} has the potential to enhance the trustworthiness and reliability of these transformative technologies.
